Revisiting Boustrophedon Coverage Path Planning as a Generalized Traveling Salesman Problem

In this paper, we present a path planner for low-altitude terrain coverage in known environments with unmanned rotary-wing micro aerial vehicles (MAVs). Airborne systems can assist humanitarian demining by surveying suspected hazardous areas (SHAs) with cameras, ground-penetrating synthetic aperture radar (GPSAR), and metal detectors. Most available coverage planner implementations for MAVs do not consider obstacles and thus cannot be deployed in obstructed environments. We describe an open source framework to perform coverage planning in polygon flight corridors with obstacles. Our planner extends boustrophedon coverage planning by optimizing over different sweep combinations to find the optimal sweep path, and considers obstacles during transition flights between cells. We evaluate the path planner on 320 synthetic maps and show that it is able to solve realistic planning instances fast enough to run in the field. The planner achieves 14% lower path costs than a conventional coverage planner. We validate the planner on a real platform where we show low-altitude coverage over a sloped terrain with trees.

==> Makefile <==
# The target that we want to build, TODO: change name if required
targets=main.pdf

# Dependencies, all files which are taken into consideration when make decides
# if rebuilding is necessary
deps=$(wildcard */*.tex) $(wildcard figures/*.png) $(wildcard figures/*.jpg) \
	$(wildcard figures/*.jpeg) $(wildcard figures/*.pdf) \
	$(wildcard *.bib)

# NOTE: you should not change anything below
%.pdf: %.tex $(deps) Makefile build
	# cd to build and build the report
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex $<
	cd build && BIBINPUTS=../:${BIBINPUTS} BSTINPUTS=../:${BSTINPUTS} bibtex $*
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex $<
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS} pdflatex $<
	# copy the resulting pdf back to the main directory (mv is no good, because
	# make will rebuild even if nothing has changed)
	cp build/$@ .

all: $(targets)

clean: buildclean

build:
	# make sure that build exists
	mkdir -p build

buildclean:
	# remove the build folder
	rm -rf build *~ */*~

distclean: clean
	# remove the build folder (clean) and the target pdf
	rm -f $(targets)

installdeb:
	# required packages to use this makefile
	sudo apt-get install texlive texlive-math-extra texlive-publishers

.PHONY: clean buildclean distclean all dist installdeb


==> figures/iterative_approximation.tex <==
\begin{algorithm}
\caption{Iterative Variational Shape Approximation} \label{lst:iterative_approximation}
\begin{algorithmic}[1]
  \Require $\mathrm{mesh}$, $\mathrm{sensor\_model}$
  \State $\mathrm{approximation}.\textproc{setInitialSeed()}$
  \State $\mathrm{approximation}.\textproc{runVSA()}$
  \While {$\mathrm{approximation}.\textproc{cover()}$}
  \EndWhile


  \State $\mathrm{simple\_segments}[] = \textproc{SegmentMap}(\mathrm{mesh})$
  \State $\mathrm{trajectories}[][] = \textproc{GenerateTrajectories}(\mathrm{simple\_segments}, \newline
  ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \mathrm{sensor\_settings})$
  \State $\mathrm{path}[] = \textproc{GenerateCoveragePath}(\mathrm{trajectories}, \mathrm{start}, \mathrm{goal})$
  \State \Return $\mathrm{path}$
\end{algorithmic}
\end{algorithm}

